Electronic states of multilayer VTe2: quasi-one-dimensional Fermi surface and implications to charge-density waves

We have performed angle-resolved photoemission spectroscopy on epitaxial VTe2 films to elucidate the relationship between the fermiology and charge-density waves (CDW). We found that a two-dimensional triangular pocket in 1 monolayer (ML) VTe2 is converted to a strongly warped quasi-one-dimensional (1D) Fermi surface in the 6ML counterpart, likely associated with the 1T-to-1T' structural phase transition. We also revealed a metallic Fermi edge on the entire Fermi surface in 6ML at low temperature distinct from anisotropic pseudogap in 1ML, signifying a contrast behavior of CDW that is also supported by first-principles band-structure caluculations. The present result points to the importance of simultaneously controlling the structural phase and fermiology to manipulate the CDW properties in ultrathin transition-metal dichalcogenides.

==> tex_rev2(kawakami)_0706_double_PM15/acknowledment.tex <==
\begin{acknowledgments}
We thank K. Horiba and H. Kumigashira for their assistance in the ARPES experiments. This work was supported by JST-CREST (No. JPMJCR18T1), JST-PREST (No. JPMJPR20A8), JSPS KAKENHI Grants (Nos. JP18H01821, JP18H01160 and JP17H01139), KEK-PF (Proposal No. 2018S2-001), Science research projects from Shimazu Science Foundation, World Premier International Research Center, Advanced Institute for Materials Research. T. Kawakami and T. Kato acknowledge support from GP-Spin at Tohoku University.
\end{acknowledgments}
